Removal of Quantifiers by Elimination of Boundary Points

We consider the problem of elimination of existential quantifiers from a Boolean CNF formula. Our approach is based on the following observation. One can get rid of dependency on a set of variables of a quantified CNF formula F by adding resolvent clauses of F eliminating boundary points. This approach is similar to the method of quantifier elimination described in [9]. The difference of the method described in the present paper is twofold: {\bullet} branching is performed only on quantified variables, {\bullet} an explicit search for boundary points is performed by calls to a SAT-solver Although we published the paper [9] before this one, chrono- logically the method of the present report was developed first. Preliminary presentations of this method were made in [10], [11]. We postponed a publication of this method due to preparation of a patent application [8].

==> support.tex <==
%
% remark: confession
%
\begin{remark}
\label{rem:confession}
In the FMCAD submission, we used the notion of locally redundant variables (Definition~\ref{def:loc_red_vars}).
This needs to be corrected. Definition~\ref{def:loc_red_vars} should be replaced with 
Definition~\ref{def:glob_red_vars} of globally redundant variables. (So it is a very easy fix). The reason
is as follows.  Let D-sequents \Dss{F}{q_1}{X'} and \Dss{F}{q_2}{X'} be resolvable on variable $x$ and
D-sequent \Dss{F}{q}{X'} be their resolvent. Let \Su{X^1}{red}, \Su{X^2}{red} and \Su{X}{red} be the subset of
 variables of $X$ already proved redundant in \cof{F}{q_1}, \cof{F}{q_2} and \cof{F}{q} respectively.
From the fact that  $X'$ is locally redundant in \DDis{F}{q_1}{\Su{X^1}{red}} and 
in \DDis{F}{q_2}{\Su{X^2}{red}} one can only derive that $X'$ is \ti{globally} redundant in 
\DDis{F}{q}{\Su{X}{red}} (in general, $X'$ is not locally redundant in \DDis{F}{q}{\Su{X}{red}}). In other words,
Proposition~\ref{prop:res_rule} (that resolving  D-sequents is sound) is true only in terms of global redundancy
of variables.


Note that this does not affect  Proposition~\ref{prop:correctness} (about the correctness of \Di\!\!).
However, the proof of Proposition~\ref{prop:correctness}  holds only if 
the notion of global redundancy of variables is used. 
As we already mentioned above, to fix the situation one just needs to replace Definition~\ref{def:loc_red_vars}
with Definition~\ref{def:glob_red_vars}. Such replacement does not affect 
propositions and their proofs if they are correct
in terms of local redundancy of variables (because local redundancy is a 
special case of global redundancy, see Lemma~\ref{lemma:special_case}). 
 For the rest of the Appendix if we do not say what kind of redundancy
is meant we assume that it is global redundancy (Definition~\ref{def:glob_red_vars}).
-------------
%
% example
%
\begin{example}
Let CNF formula $F(X,Y)$ where $X =\{x_1,x_2\}$, $Y=\{y_1,y_2\}$
consist of two clauses: $C_1=x_1 \vee \overline{x}_2 \vee y_1$ and $C_2=\overline{x}_1 \vee x_2 \vee y_2$.
Let $\Su{X}{red}= \emptyset$.
Suppose that assignment $x_1 = 0$ is made. Then the formula \cof{F}{q} where $\pnt{q}=(x_1=0)$ is
equal to $\overline{x}_2 \vee y_1$. (The clause $C_2$ is satisfied by \pnt{q}). 
Note that variable $x_2$ is monotone in \cof{F}{q} and so it is redundant 
there (due to Proposition~\ref{prop:mon_var_red}).
Hence, the D-sequent $(F,\pnt{q}) \rightarrow \s{x_2}$ holds.
\end{example}
----------------
\begin{proposition}
%\label{prop:form_replacement}
Let $F^+(X,Y)$ be a CNF formula obtained from $F(X,Y)$ by adding some resolvents of clauses of $F$.
Let \pnt{q} be a partial assignment to variables of $X$ and $X' \subseteq X$.
Denote by $\Su{X}{red}$ the set of variables of $X$ already proved redundant for \cof{F}{q}. 
Then the fact that D-sequent \Dss{F}{\Su{X}{red}}{q}{X'} holds implies that
\Dss{F^+}{\Su{X}{red}}{q}{X'} holds too. The opposite is not true.
\end{proposition}
\begin{mmproof}
First, let us prove that if  \Dss{F}{\Su{X}{red}}{q}{X'} holds, \Dss{F^+}{\Su{X}{red}}{q}{X'} does too.
(In this proof, we assume that the replacement of $F$ with $F^+$ takes place only in one D-sequent.
However, Proposition~\ref{prop:form_replacement} can be also used to prove that such a replacement 
can be performed in all the derived D-sequents simultaneously.
See Remark~\ref{rem:replace_all} below.)

Let us assume the contrary, i.e. \Dss{F}{\Su{X}{red}}{q}{X'} holds but \Dss{F^+}{\Su{X}{red}}{q}{X'} does not.
According to Definition~\ref{def:d_sequent}, this means  that variables of $X'$ are not
 redundant in \DDis{F^+}{q}{\Su{X}{red}}
while they are redundant in \DDis{F}{q}{\Su{X}{red}}. Then 
there is a point \pnt{p} that is an $X'$-removable point of \DDis{F^+}{q}{\Su{X}{red}}
 but is not an $X'$-removable point  of \DDis{F}{q}{\Su{X}{red}}.
Let us consider the  three reasons  for \pnt{p} not to be an $X'$-removable boundary point of \DDis{F}{q}{\Su{X}{red}}.
\begin{itemize}
%item
\item \pnt{p} satisfies \DDis{F}{q}{\Su{X}{red}}. Then it also satisfies \DDis{F^+}{q}{\Su{X}{red}}
 and hence cannot be a boundary point of \DDis{F^+}{q}{\Su{X}{red}}. Contradiction.
%item
\item \pnt{p} is not  an $X^*$-boundary point of \DDis{F}{q}{\Su{X}{red}}
 where $X^* \subset X'$. That is \pnt{p} falsifies a  clause of $C$
              of \DDis{F}{q}{\Su{X}{red}} that does not contain a variable of $X'$. Since  
\DDis{F^+}{q}{\Su{X}{red}} also contains $C$, point \pnt{p} cannot
              be an $X^*$-boundary point of \DDis{F^+}{q}{\Su{X}{red}} either. Contradiction.
%
\item \pnt{p} is an $X^*$-boundary point of \DDis{F}{q}{\Su{X}{red}} but is not $X'$-removable.
 This means that one can  obtain a point \pnt{p^*}   satisfying \DDis{F}{q}{\Su{X}{red}} by flipping 
the values of variables of $X'$ in \pnt{p}. Since \pnt{p^*} also satisfies \DDis{F^+}{q}{\Su{X}{red}},
one has to conclude that \pnt{p} is not an $X'$-removable point of \DDis{F^+}{q}{\Su{X}{red}} either. Contradiction.
\end{itemize}
%
\vspace{10pt}
Now we show that if $(F^+,\pnt{q}) \rightarrow X'$ holds this does not mean that 
 $(F,\pnt{q}) \rightarrow X'$ does. 
Let $F(X,Y)$ be a CNF formula where $X=\s{x}, Y=\s{y}$. Let $F$ consist of clauses $C_1$,$C_2$
 where $C_1=x \vee y$ and $C_2 =\overline{x} \vee y$.
Let $F^+$ be obtained from $F$ by adding the unit clause $y$ (that is the resolvent of $C_1$ 
and $C_2$). It is not hard to see
that the D-sequent $(F^+,\emptyset)~\rightarrow~\s{x}$ holds. ($F^+$ does not 
have any \s{x}-boundary points. Hence it cannot have
an \s{x}-removable boundary point.) At the same time, $F$ has an \s{x}-removable boundary point 
\pnt{p}=($x$=0,$y$=0). So the D-sequent
  $(F,\emptyset) \rightarrow \s{x}$ does not hold.
\end{mmproof}
%
%  remark
%
\begin{remark}
\label{rem:replace_all}
Let $F(X,Y)$ be a CNF formula and $S_1,\ldots,S_k$  be a set of D-sequents
numbered in the order they are derived where $S_i = \Dss{F_k}{X^*_k}{q_k}{X_k}$. Here we assume that
$F_1$ is the formula $F$ itself and  $F_j$ can be obtained from $F_i$, $i < j$ by adding some resolvent-clauses of $F_i$.
One can use Proposition~\ref{prop:form_replacement}  to show that it is correct to simultaneously
perform the $k$ replacements where in each D-sequent $S_i$ formula $F_i$ is replaced with $F^+$.
The idea is to use induction on $k$. The base statement is that
replacing $F_1$ with $F^+$ holds for $S_1$. This is true due to Proposition~\ref{prop:form_replacement}.
The induction step is to show that $S_{i+1}$ holds after replacing $F_{i+1}$ with $F^+$ assuming that  
$S_1,\ldots,S_i$ hold after such a replacement. The induction step is also correct due to Proposition~\ref{prop:form_replacement}.
\end{remark}
------------------
\begin{proposition}
%\label{prop:many_vars_elim}
Let $F(X,Y)$ be a CNF formula. Let $X'$ be the redundant variables of $F$ where
$X' \subseteq X$.  Then each $X$-removable boundary point \pnt{p}  of $F$ can be eliminated by a clause
$C$, $\V{C} \subseteq Y$ derived from non-$X'$-clauses of $F$.
\end{proposition}
\begin{mmproof}
Let \pnt{p} be an $X$-removable boundary point of $F$.  Let $P$ be the set of $2^{|X|}$ points that consists  of \pnt{p}
and all the points that can be obtained from \pnt{p} by flipping variables of $X$. Since \pnt{p} is $X$-removable,
every point of $P$ falsifies $F$.
Assume that  $\pnt{p^*} \in P$ is an $X'$-boundary point. Since 
all $X'$-neighbors of \pnt{p^*} are unsatisfying assignments (because they form a subset of $P$), one has
to conclude that \pnt{p^*} an $X'$-removable boundary point of $F$. We have a contradiction, which means
that \pnt{p^*} falsifies at least one clause of $F$ that does not have any variables of $X'$. Let $G(X,Y)$
be a subset of non-$X'$-clauses of $F$ such that for every point \pnt{p^*} of $P$ there is a clause
of $G(X,Y)$ falsified by \pnt{p^*}. Then there is a clause $C(Y)$ consisting of the literals of $Y$ falsified
by \pnt{p} that is implied by $G$ and hence can be derived from $G$ by resolution.
\end{mmproof}
--------------------
%
%    Main lemma
%
\begin{lemma}
\label{lemma:main}
Let $\exists{X}.F(X,Y) \equiv F^*(Y)$. Let  \pnt{x} and \pnt{y} be assignments
to variables of $X$ and $Y$ respectively.
Then 
\begin{description}
\item[a)] $F^*$(\pnt{y})=1 $\rightarrow$ $\exists$\pnt{x},$F$(\pnt{x},\pnt{y})=1
\item[b)] $F^*$(\pnt{y})=0 $\rightarrow$ $\forall$\pnt{x},$F$(\pnt{x},\pnt{y})=0
\end{description}
\end{lemma}
\begin{mmproof}
Trivially follows from  $\exists{X}.F(X,Y) \equiv F^*(Y)$.
\end{mmproof}
\vspace{8pt}
-----------------
\begin{example}
Let CNF formula $G(Z)$ consist of the following four clauses:
$C_1 = z_1 \vee z_2$, $C_2= \overline{z}_1 \vee z_3$, $C_3~=~\overline{z}_2~\vee~z_4$, $C_4=\overline{z}_3 \vee \overline{z}_4$.
In the branch $z_4=0$, clause $C_4$ is satisifed which makes variable $z_3$ monotone and hence redundant. So $\pnt{q'}=(z_4=0)$,
\Su{Z}{red} = \s{z_3} and \DDis{F}{q'}{\Su{Z}{red}} =  $(z_1 \vee z_2) \wedge \overline{z}_2$. Variable $z_1$ is monotone
in \DDis{F}{q'}{\Su{Z}{red}}  and so  D-sequent \DDs{G}{\s{z_3}}{q'}{z_1} can be derived. Note that since  $z_1$ is 
monotone, from Lemma~\ref{lemma:mon_loc_red} it follows that $z_1$ is  locally redundant in \DDis{F}{q'}{\Su{Z}{red}}. 

In the branch $z_4=1$, clause $C_3$ is satisifed which makes variable $z_2$ monotone and hence redundant. So $\pnt{q''}=(z_4=1)$,
\Su{Z}{red} = \s{z_2} and \DDis{F}{q''}{\Su{Z}{red}} =  $(\overline{z}_1 \vee z_3) \wedge \overline{z}_3$. Variable $z_1$ is monotone
in \DDis{F}{q''}{\Su{Z}{red}}  and so  D-sequent \DDs{G}{\s{z_2}}{q''}{z_1} can be derived. Note  that again since  $z_1$ is 
monotone, from Lemma~\ref{lemma:mon_loc_red} it follows that $z_1$ is  locally redundant in \DDis{F}{q''}{\Su{Z}{red}}.

By resolving D-sequents  \DDs{G}{\s{z_3}}{q'}{z_1} and \DDs{G}{\s{z_2}}{q''}{z_1} on variable $z_4$, one
produces D-sequent $(G,\emptyset,\emptyset) \rightarrow \s{z_1}$ . Note however, that in this D-sequent, variable $z_1$ is \ti{globally}
redundant. Indeed, let us consider, for instance, the point \pnt{p'}= ($z_1=0$, $z_2=0$, $z_3=0$, $z_4=0$). Since \pnt{p'} falsifies
only the clause $C_1$ of $F$, it is a \s{z_1}-boundary point. By flipping the value of $z_1$ in \pnt{p'} one obtains
the point \pnt{p''} falisfying only the clause $C_2$. So \pnt{p''} is also a \s{z_1}-boundary point. So by changing only the
value of \pnt{z_1} one cannot obtain a satisfying assignment from \pnt{p'} and hence to show that the latter is not
removable. A satisfying assignment ($z_1=0$, $z_2=1$, $z_3=0$, $z_4=1$) can be obatined from \pnt{p'} by flipping the values of $z_2$ and $z_4$.
So $z_1$ is redundant only globally.
\end{example}
--------------
%
%  Lemma
%
\begin{lemma}
\label{lemma:merging_red_vars1}
Let $F(X,Y)$ be a CNF formula and \pnt{q} be a partial assignment to variables of $X$.
Let $X'$ be  the subset of variables of $X$ already proved redundant in \cof{F}{q}.
Let D-sequent \Dss{F}{X'}{q}{X''}  be derived.
Then the variables of $X' \cup  X''$ are redundant in \cof{F}{q}.
\end{lemma}
\begin{mmproof}
Denote by $X^*$ the set $X' \cup X''$. Assume the contrary. Let D-sequent   \Dss{F}{X'}{q}{X''} hold and there is a removable
$X^+$-boundary point \pnt{p}  of \cof{F}{q} where $X^+ \subseteq X^*$. Let us consider the two possible cases:
\begin{itemize}
\item  $X^+ \subseteq X'$ (and so $X^+ \cap X'' = \emptyset$).
Since \pnt{p} is removable, the variables of $X'$ cannot be redundant in \cof{F}{q} and so \Dss{F}{X'}{q}{X''}  does not hold.
Contradiction.
\item  $X^+ \not\subseteq X'$ (and so $X^+ \cap X'' \neq \emptyset$). 
 Then \pnt{p} is an $X''^+$-boundary
 point of \DDis{F}{q}{X'} where $X''^+ = X^+ \cap X''$. 
Indeed, for every variable $x$ of $X^+$ there has to be a clause  $C$ of \cof{F}{q} 
falsified by \pnt{p} such that $\V{C}~\cap X^+~=~\s{x}$.
 Otherwise, $x$ can be removed from $X^+$, which contradicts the assumption that \pnt{p} is an $X^+$-boundary point.
 This means that for every variable $x$ of $X''^+$ there is a clause $C$ falsified by \pnt{p} such 
that $\V{C}~\cap X''^+~=~\s{x}$. 

\vspace{10pt}
Let $P$ denote the set of all $2^{|X \setminus (\mi{Vars}(\boldsymbol{q}) \cup X')|}$ points obtained from \pnt{p} by flipping 
values of variables of $X \setminus (\Va{q} \cup X')$.
Let us consider the following two possibilities.
     \begin{itemize}
        \item Every point of $P$ falsifies \DDis{F}{q}{X'}. This means that the point \pnt{p}
           is a removable $X''^+$-
               boundary point of \DDis{F}{q}{X'}. Hence the variables of $X''$ are not redundant in \DDis{F}{q}{X'},
 which contradicts  the fact that the D-sequent \Dss{F}{X'}{q}{X''} holds.
         \item A point \pnt{d} of $P$ satisfies \DDis{F}{q}{X'}. Let us consider the following two cases.
            \begin{itemize}
              \item \pnt{d} satisfies \cof{F}{q}. This contradicts the fact that \pnt{p} is
 an removable $X^+$-boundary point of \cof{F}{q}.
                      (By flipping variables of $X \setminus \Va{q}$
                       one can  obtain a point satisfying \cof{F}{q}.)

              \item \pnt{d} falsifies some clauses of \cof{F}{q}. Since \cof{F}{q} and \DDis{F}{q}{X'}
 are different only in $X'$-clauses,
                            \pnt{d} is an $X'^*$-boundary point of \cof{F}{q} where $X'^* \subseteq X'$. Since
 \pnt{p} is a removable $X^+$-boundary point
                            of \cof{F}{q}, \pnt{d} is a removable  $X'^*$-boundary point of \cof{F}{q}.
 This contradicts the fact that the variables of $X'$ are redundant in \cof{F}{q}.
            \end{itemize}
     \end{itemize}
\end{itemize}
\end{mmproof}

